Design Methodology of Hydraulically-driven Soft Robotic Gripper for a Large and Heavy Object

This paper presents a design methodology of a hydraulically-driven soft robotic gripper for grasping a large and heavy object -- approximately 10 - 20 kg with 20 - 30 cm diameter. Most existing soft grippers are pneumatically actuated with several hundred kPa pressure, and cannot generate output force sufficient for such a large and heavy object. Instead of pneumatic actuation, hydraulic actuation has a potential to generate much larger power by several MPa pressure. In this study, we develop a hydraulically-driven soft gripper, in which its basic design parameters are determined based on a mathematical model that represents the relationship among the driving pressure, bending angle, object mass and grasping force. Moreover, we selected materials suitable for grasping a heavier object, based on the finite element analysis result of the detailed design. We report experimental results on a 20 kg object grasping and closed-loop control of the finger bending angle.

==> grasping_flexibility.tex <==
\begin{figure}[t]
    \centering
    \subfigure[Grasping 2kg weight object]{
	\includegraphics[width=0.28\hsize]{figure/control/2kg_grasping.eps}}
    \subfigure[Apply external force]{
	\includegraphics[width=0.28\hsize]{figure/control/2kg_grasping_disturb.eps}}
    \subfigure[Finger angle graph]{
	\includegraphics[width=0.45\hsize]{figure/control/finger_control_angle.eps}}
    \subfigure[Pressure graph]{
	\includegraphics[width=0.45\hsize]{figure/control/finger_control_pressure.eps}}
    \caption{Experiment of grasping a 2 kg object by controlling the average bending angle of the four fingers to 50 degrees. After about 5 seconds from the start of the pressurization, an external force was applied to the grasped object as shown in (b). The bending angle of each finger is shown in (c), and the driving pressure is shown in (d).\label{fig:finger_control}}
\end{figure}

%4本のフィンガの屈曲角度の平均値が50度になるように制御を行い，2kgの物体を把持した様子を図 \ref{fig:finger_control} (a)に示す．このとき，加圧開始から約5秒経過後に図 \ref{fig:finger_control} (b)のように把持物体に外力を加えた．その時の各フィンガの屈曲角度を図 \ref{fig:finger_control} (c)に，駆動圧力を図 \ref{fig:finger_control} (d)に示す．まず，外力を加える前の区間(i)に注目すると，フィンガの平均値がおよそ50度に制御できていることが分かる．次に，外力を加えている区間(ii)に注目すると，区間(i)に比べて駆動圧力が小さくなっていることが読み取れる．このことから，角度制御を行った際の外力に対するハンドの把持柔軟性について考察する．
Fig. \ref{fig:finger_control} (a) shows an experiment where a 2 kg object is grasped using closed-loop control with $\theta_{ref}=$ 50 degrees. To test robustness, we applied an external force to the object about 5 seconds after the start of the grasp, as illustrated in Fig. \ref{fig:finger_control} (b). Fig. \ref{fig:finger_control} (c) displays the bending angle of each finger, and Fig. \ref{fig:finger_control} (d) shows the driving pressure. Initially, in state (i) before the external force is applied, the average finger angle is controlled to approximately 50 degrees. In state (ii), when the external force is applied, the driving pressure is lower than in state (i). This result demonstrates the flexibility of the gripper in adjusting to external forces while maintaining angle control.

%(a)物体に外力が加わっていない場合，(b)圧力制御を行い外力を加えた場合，(c)角度制御を行い外力を加えた場合の把持力をそれぞれ計算する．(a)(b)(c)それぞれの場合の駆動圧力と屈曲角度$P_a, \theta_a, P_b, \theta_b, P_c, \theta_c$はFig. \ref{fig:finger_control} (c)(d)より，Table. \ref{tb:finger_control_disturbance}と読み取れる．ここで，(b)の場合には，圧力が外力を加える前後で変わらないとし，角度は角度制御を行った場合と同じ角度で屈曲すると仮定した．この時，(a)(b)(c)それぞれの場合の把持力はTable. \ref{tb:finger_control_disturbance}のように計算できる．この結果から，フィンガを角度制御した場合に，圧力制御に比べて，外力に対する反力が0.29kgf低いことが分かる．ここで，リジットなロボットハンドでは，一般的にフィンガの角度制御を行った場合には，その位置を維持しようとするために，外力に対する反力が大きくなる．一方で，各フィンガの流路が同じであるソフトハンドでは，フィンガを角度制御することで，外力に対する把持柔軟性も得られることを確認した．

\subsection{Evaluation of Flexibility to External Force}
In general, closed-loop control typically increases finger stiffness, reducing flexibility. To assess the flexibility achieved with the closed-loop control described, we compare the grasping force under three conditions:
\begin{enumerate}[label=Condition~\Alph*, leftmargin=*]
    \item Grasping force under closed-loop control without any external force. This force is estimated from the pressure $P_a$ and angle $\theta_a$ during period (i) in Figs. \ref{fig:finger_control} (c) and \ref{fig:finger_control} (d).
    \item Grasping force under closed-loop control with an external force applied. This force is estimated from the pressure $P_b$ and angle $\theta_b$ during period (ii) in Figs. \ref{fig:finger_control} (c) and \ref{fig:finger_control} (d).
    \item Grasping force under pressure control with an external force applied. This force is estimated from the angle $\theta_c$ during period (ii) in Fig. \ref{fig:finger_control} (c), assuming that the pressure $P_c$ remains constant, as pressure control maintains a steady pressure.
\end{enumerate}

Table \ref{tb:finger_control_disturbance} shows the estimated grasping forces for each condition. The estimated values are 0.61 kgf for Condition A, 0.53 kgf for Condition B, and 0.82 kgf for Condition C. Thus, the grasping force in Condition B (closed-loop control) is 0.29 kgf lower than in Condition C, indicating that Condition B provides higher flexibility against external forces. This finding contrasts with the typical characteristics of closed-loop and pressure control systems—where closed-loop control generally increases stiffness, and pressure control enhances flexibility.

The observed increased flexibility in Condition B can be attributed to the closed-loop control mechanism, which regulates the average bending angle of the fingers connected through a single flow path. For instance, in Fig. \ref{fig:finger_control} (b), the left finger's displacement to the left in response to the external force caused a reduction in its bending angle. Consequently, the control system adjusted the bending angle of the right finger to compensate, increasing its angle. This adaptive control strategy enhances the fingers' ability to accommodate external disturbances.

\begin{table}[t]
    \centering
    \footnotesize
        \caption{\footnotesize{Difference in gripping force of fingers according to the difference in control.}}
    \begin{tabular}{ccc|ccc}
        Condition & Control type & External force & Pressure & Angle & Grasping force \rule[-7pt]{0pt}{14pt} \\ \hline
        A & Closed-loop & -- & 0.89 MPa & 50 deg & 0.61 kgf \rule[-7pt]{0pt}{14pt} \\
        B & Closed-loop & \checkmark & 0.79 MPa & 45 deg & 0.53 kgf \rule[-7pt]{0pt}{14pt} \\
        C & Pressure control & \checkmark & 0.89 MPa & 45 deg & 0.82 kgf \rule[-7pt]{0pt}{14pt} \\
    \end{tabular}
    \label{tb:finger_control_disturbance}
\end{table}
